Feature Selection using Stochastic Gates

Feature selection problems have been extensively studied for linear estimation, for instance, Lasso, but less emphasis has been placed on feature selection for non-linear functions. In this study, we propose a method for feature selection in high-dimensional non-linear function estimation problems. The new procedure is based on minimizing the $\ell_0$ norm of the vector of indicator variables that represent if a feature is selected or not. Our approach relies on the continuous relaxation of Bernoulli distributions, which allows our model to learn the parameters of the approximate Bernoulli distributions via gradient descent. This general framework simultaneously minimizes a loss function while selecting relevant features. Furthermore, we provide an information-theoretic justification of incorporating Bernoulli distribution into our approach and demonstrate the potential of the approach on synthetic and real-life applications.

==> latex-headers.tex <==
\usepackage{color}
\usepackage{colortbl}
\usepackage{lmodern}
\usepackage{bbm}
\usepackage{subfigure}
\usepackage{graphicx}
\usepackage{amsthm}
\usepackage{wasysym}
\usepackage{fdsymbol}
\usepackage{rotating}
\usepackage{algorithmic}
\usepackage[algoruled,vlined]{algorithm2e}
\usepackage{booktabs}
\usepackage{media9}
\usepackage{animate}
\usepackage{picture}
\usepackage{adjustbox}
\usepackage{multirow}
\usepackage{hhline}

\usepackage{tikz}
\usetikzlibrary{shapes.arrows}
\usetikzlibrary{decorations.pathmorphing}

\DeclareMathOperator{\proj}{proj}
\newcommand{\abs}[1]{\left | #1 \right |}
\newcommand{\norm}[1]{\left \| #1 \right \|}
\newcommand{\norminline}[1]{\| #1 \|}
\newcommand{\inprod}[2]{\left \langle #1, #2 \right \rangle}
\newcommand{\inprodinline}[2]{\langle #1, #2 \rangle}
\DeclareMathOperator{\spn}{span}
\DeclareMathOperator{\tr}{tr}
\newcommand{\transpose}[1]{#1^T}
\newtheorem{proposition}{Proposition}

\usepackage[absolute,overlay]{textpos}
\usepackage{ifthen}
\usepackage{svg}

\usepackage{xmpmulti} %for animation

\newcommand {\myvec}[1] {{\mbox{\boldmath $#1$}}}
\newcommand{\myx}{\myvec{x}}
\newcommand{\myz}{\myvec{z}}
\newcommand{\myth}{\myvec{\theta}}
\newcommand{\mys}{\myvec{s}}
\newcommand{\tils}{\tilde{S}}
\newcommand{\prob}{\mathbb{P}}
\newcommand{\reals}{\mathbb{R}}


==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    if (!($root_filename eq $_[0]))
    {
        system( "latexmk -pdf \"$_[0]\"" );
    }
}
